Synchronizing Automata: Open Problems

We survey selected open problems in the theory of synchronizing automata, centered around the famous \v{C}ern\'y conjecture. A deterministic finite automaton is called synchronizing if it admits a reset word whose action maps all states to a single state. The \v{C}ern\'y conjecture states that every synchronizing automaton with $n$ states possesses a reset word of length at most $(n-1)^2$. We discuss avoiding words, compressing a state with another, synchronization of a (given or any) subset, complexity of deciding the synchronizability, average reset threshold, and linear-algebraic methods. Some new auxiliary results are also presented.

==> eptcsdata.tex <==
\providecommand{\firstpage}{33}
\providecommand{\publicationstatus}{M. Hospod\'ar et al. (Eds.): 17th International Conference \\on Automata and Formal Languages (AFL 2026)\\
EPTCS 451, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.451.3}{10.4204/EPTCS.451.3}}
\pdfoutput=1

